L-Shape based Layout Fracturing for E-Beam Lithography

Layout fracturing is a fundamental step in mask data preparation and e-beam lithography (EBL) writing. To increase EBL throughput, recently a new L-shape writing strategy is proposed, which calls for new L-shape fracturing, versus the conventional rectangular fracturing. Meanwhile, during layout fracturing, one must minimize very small/narrow features, also called slivers, due to manufacturability concern. This paper addresses this new research problem of how to perform L-shaped fracturing with sliver minimization. We propose two novel algorithms. The first one, rectangular merging (RM), starts from a set of rectangular fractures and merges them optimally to form L-shape fracturing. The second algorithm, direct L-shape fracturing (DLF), directly and effectively fractures the input layouts into L-shapes with sliver minimization. The experimental results show that our algorithms are very effective.

==> doc/introduction__Bei_Yu_s_conflicted_copy_2014-01-23_.tex <==

\vspace{-.1in}
\section{Introduction}

E-Beam lithography (EBL) \cite{EBL_SPIE05_Pain} is widely deployed in the mask manufacturing,
which is a significant step affecting the fidelity of the printed image on the wafer and critical dimension (CD) control.
Because of the capability of accurate pattern generation, EBL is also a promising candidates for sub-22nm logic nodes,
along with extreme ultra violet (EUV) \cite{EUV_SPIE2010_Arisawa} and double/multiple patterning lithography (DPL/MPL) \cite{DPL_ICCAD08_Kahng}\cite{TPL_ICCAD2011_Yu}.
%EBL has been used in small volume LSI production and R\&D to develop the technological nodes ahead of mass production.
For EBL writing, a fundamental step is \textit{layout fracturing}, where the layout pattern is decomposed into numerous non-overlapping rectangles.
Subsequently the layout is prepared and exposed by an EBL writing machine onto the mask or the wafer,
where each fractured rectangle is shot by one variable shaped beam (VSB).

% Cost increasing of mask writing
As the minimum feature size further decreases, the number of rectangles in the layout is steadily increased.
First, longer writing time and larger data volume are caused by highly complex optical proximity correction (OPC).
%reticle enhancement technique (RET) that is used to optimize mask apertures for the manufacture of deeply sub-wavelength features.
Besides, the introduction of advanced lithographic techniques, e.g., DPL/MPL, add more masks in the mask manufacturing.
Since the manufacturing cost is directly associated with increasing write time and data volume, the cost is also steadily increased.
In addition, the low throughput has been and is still the bottleneck of EBL writing.
%At sub-22nm logic nodes, the number of shots after fracturing may be too large to be practically written by EBL.

To overcome this manufacturing problem, several optimization methods have been proposed to reduce the EBL writing time to a reasonable level
\cite{EBL_SPIE2010_Sahouria}\cite{EBL_SPIE2011_Elayat}\cite{EBL_TCAD2012_Yuan}.
%These optimization methods contain both hardware improvement and software speed-up
%i.e., jog alignment, multi-resolution writing, character projection, and L-shape shot
Among them, the L-shape shot strategy is a very simple yet effective approach to reduce the e-beam mask writing time,
and thus reduce the mask manufacturing cost and improve the throughput
\cite{EBL_SPIE2010_Sahouria}\cite{EBL_SPIE2011_Elayat}.
Besides, this technique can be also applied to reduce the cost of lithographic process.
The conventional EBL writing is based on rectangular VSB shots.
As illustrated in Fig. \ref{fig:EBL}(a), the electrical gun generates an initial beam, which becomes uniform through the shaping aperture.
Then the second aperture finalizes the target shape with a limited maximum size.
As an improved technique, the printing process of the L-shape shot is illustrated in Fig. \ref{fig:EBL}(b).
One additional aperture, the third aperture, is employed to create L-shape shots.
To take advantage of this new printing process, new fracturing methodology is needed to provide L-shape in the fractured layout.
%With careful design, we can see that the
L-shape shot strategy has the potentiality to reduce the EBL writing time or cost by 50\% if all rectangles are combined into L-shapes.
For example in Fig. \ref{fig:example}, instead of four rectangles,
using L-shape fracturing only requires two L-shape shots.

%Besides, until now there is no known mask writer format or methodology has a mechanism to describe the L-shape based fracturing.
%The limiting factor in the implementation of this technology is the development of a write tool with the additional aperture required to create L-shaped shots and the respective changes to data format and mask writer software to support it.

\begin{figure}[bt]
  \centering
  \hspace{-.1in}
  \subfigure[]{\includegraphics[width=0.23\textwidth]{shotR}}
  \hspace{-.1in}
  \subfigure[]{\includegraphics[width=0.23\textwidth]{shotL}}
  \hspace{-.1in}
  \caption{~(a) Traditional rectangular EBL writing process.~(b) L-shape writing process with one additional aperture.}
  \label{fig:EBL}
  \vspace{-.1in}
\end{figure}

\begin{figure}[bt]
  \centering
  \subfigure[]{
    \includegraphics[width=0.15\textwidth]{MergeGraph1}
  }
  \hspace{.1in}
  \subfigure[]{
    \includegraphics[width=0.15\textwidth]{MergeGraph4}
  }
  \caption{Examples of polygon fracturing.~(a) Rectangular shots with 4 shot number.~(b) L-shape shots with 2 shot number.}
  \label{fig:example}
  \vspace{-.1in}
\end{figure}

Note that the layout fracturing problem is different from the general polygon decomposition problem in geometrical science.
In order to consider yield control and CD control,
the minimum width of each shot should be above a certain threshold value $\epsilon$.
A shot whose minimum width is $< \epsilon$ is called a \textit{sliver}.
In the layout fracturing, sliver minimization is an important objective \cite{EBL_SPIE04_Kahng}.
As shown in Fig. \ref{fig:sliver}, two fractured layouts can achieve the same shot number 2.
However, because of sliver, the fractured result in Fig. \ref{fig:sliver} (a) is worse than that in Fig. \ref{fig:sliver} (b).
It shall be noted that the layout in  Fig. \ref{fig:sliver} can be written in one L-shaped shot without any sliver.

\begin{figure}[tb]
  \centering
  \vspace{-.1in}
  \subfigure[]{
    \includegraphics[width=0.18\textwidth]{sliver1}
  }
  %\hspace{-.1in}
  \subfigure[]{
    \includegraphics[width=0.18\textwidth]{sliver2}
  }
  \caption{~(a) Fracturing with one sliver.~(b) Fracturing without sliver.}
  \label{fig:sliver}
  \vspace{-.1in}
\end{figure}

% Previous Works
For traditional rectangular shots, several papers have studied the layout fracturing problem
\cite{EBL_SPIE04_Kahng}\cite{EBL_SPIE06_Kahng}\cite{EBL_SPIE08_Dillon}\cite{EBL_SPIE2011_Ma}\cite{EBL_SPIE2011_Jiang}.
Kahng et. al proposed an integer linear programming (ILP) formulation, and some matching based speed-up techniques
\cite{EBL_SPIE04_Kahng}\cite{EBL_SPIE06_Kahng}.
Recently, Ma et. al \cite{EBL_SPIE2011_Ma} presented a heuristic algorithm to generate rectangular shots and further reduce the sliver.
Compared with the rectangular fracturing problem, the L-shape fracturing problem is new and there is only limited work,
mostly describing methodology, but no systematic algorithm has been proposed so far.
\cite{EBL_SPIE2010_Sahouria} reported the initial results that L-shape fracturing can further save about 38\% of shot count, but no algorithmic details are provided.
For the general decomposition problem of polygon into L-shapes, several heuristic methods are proposed
\cite{ALG_1984_Edelsbrunner}\cite{ALG_TODAES96_Lopez}.
However, since these heuristic methods only consider horizontal decomposition, which would result in numerous slivers, 
they cannot be applied to the layout fracturing problem.

This paper presents the first systematic study for EBL L-shape fracturing considering the sliver minimization.
We propose two algorithms for the L-shape fracturing problem.
The first method, called \textit{RM}, starts from rectangles generated by any previous fracturing framework, 
and merge them into L-shapes.
A maximum weighted matching algorithm is proposed to find the optimal merging solution,
where the shot count and the sliver can be minimized simultaneously.
To further overcome the intrinsic limitations of rectangular merging,
we propose another fracturing algorithm, called \textit{DLF}.
Through effectively detect and take advantage of some special cuts,
DLF can directly fracture the layout into a set of L-shapes in $O(n^2logn)$ time.
The experimental results show that our algorithms are very promising for both shot count reduction and sliver minimization.
In addition, DLF can even achieve significant speed-up compared with previous state-of-the-art rectangular fracturing algorithm \cite{EBL_SPIE2011_Ma}.
%Compared with previous works and the rectangular merging method, DLF can not only effectively reduce the sliver length and shot number,
%but also achieve good speed-up.

\iffalse
In this paper, we present two L-shape fracturing methods.
The first method, called \textit{RM}, is a rectangular merging based incremental method.
In other words, previous rectangular fracturing algorithms can be re-used and extended.
In our second method, we propose a high performance L-shape fracturing algorithm, called \textit{DLF},
which can directly fracture a rectilinear polygon into a set of L-shapes.
Compared with previous works and the RM method, DLF can not only effectively reduce the sliver length and shot number,
but also achieve good speed-up.
Our key contributions are the following:
\begin{itemize}
  \item Propose the first systematic study for L-shape fracturing problem considering the sliver minimization;
  \item Develop a rectangular merging based method to re-use and extend previous fracturing methodology;
  \item Propose an $O(n^2logn)$ algorithm to directly fracture polygons into L-shapes;
  \item Our experimental results are very promising for both performance improvement and speed-up.
\end{itemize}
\fi

The rest of the paper is organized as follows.
Section \ref{sec:problem} presents the basics and problem formulation.
Section \ref{sec:post} provides RM, the merging based algorithm, which will also be used as a baseline.
In Section \ref{sec:algo} we propose the DLF algorithm to directly fracture polygons into L-shapes.
%Section 4 shows how we further integrate the density balance into our decomposer.
Section \ref{sec:result} presents experimental results, followed by conclusion in Section \ref{sec:conclu}.



